Consensus ADMM-Based Distributed Simultaneous Imaging & Communication

This paper takes the first steps toward enabling wireless networks to perform both imaging and communication in a distributed manner. We propose Distributed Simultaneous Imaging and Symbol Detection (DSISD), a provably convergent distributed simultaneous imaging and communication scheme based on the alternating direction method of multipliers. We show that DSISD achieves similar imaging and communication performance as centralized schemes, with order-wise reduction in computational complexity. We evaluate the performance of DSISD via 2.4 GHz Wi-Fi simulations.

==> main_results_long.tex <==
\section{Main Results}
\label{sec:results}

We begin by analyzing first-order optimality conditions in Section~\ref{subsec:results_opt_condn} to characterize the number of uplink pilots~$T_{1}$ required to solve~\eqref{prb:1}. We subsequently present the proposed DSISD algorithm in Section~\ref{subsec:results_algo}, and derive associated convergence guarantees in Section~\ref{subsec:results_algo_perf}.

\subsection{Optimality Conditions for Problem~\eqref{prb:1}}
\label{subsec:results_opt_condn}

%For analysis purposes, we focus on the \emph{unconstrained} relaxation of~\eqref{prb:1}, , with no integer constraints on uplink symbols ${X}_{T-T_{1}}$. Note that problem~\eqref{prb:1} is still non-convex without integer constraints since the objective function is bi-convex.

%\textcolor{red}{$\mathcal{L}$ is never defined. There is no need for equality inside the Lagrangian in the equations below; write the arguments.}

Let the objective function in~\eqref{prb:1} be denoted by
\begin{equation*}
    \mathcal{L}\big({f},{X}_{T-T_{1}}\big) = \frac{1}{2} \sum\limits_{n = 1}^{N} \big\|{Y}_{T}^{(n)} {-} {P}_{\mathsf{RX}}^{(n)} \mathsf{diag}\big({f}\big) \big({P}_{\mathsf{TX}} \big)^{\top} {X}_{T} \big\|_{F}^{2}. 
\end{equation*}

The KKT conditions for~\eqref{prb:1} correspond to
\begin{equation*}
    \nabla_{{f}} \mathcal{L}\big({f}^{*},{X}_{T-T_{1}}^{*} \big) = {0},~\nabla_{{X}_{T-T_{1}}} \mathcal{L}\big({f}^{*},{X}_{T-T_{1}}^{*} \big) = {0},
\end{equation*}
where ${f}^{*}$ and ${X}_{T-T_{1}}^{*}$ are minimizers of~\eqref{prb:1}. Hence, the stationary points of~\eqref{prb:1} are given by
\begin{align}
    \label{eq:opt3}
    {f}^{*} &= \big(\left.{H}_{\mathsf{img}}\right|_{{X}_{T-T_{1}} = {X}_{T-T_{1}}^{*}}\big)^{\dagger} \mathsf{vec}\big({Y}_{T}\big), \\
    \label{eq:opt4}
    {X}_{T-T_{1}}^{*} &= \big(\left.{H}_{\mathsf{comm}}\right|_{{f} = {f}^{*}}\big)^{\dagger} {Y}_{T-T_{1}},
\end{align}
where $(\cdot)^{\dagger}$ denotes the pseudo-inverse and $\mathsf{vec}(\cdot)$ denotes the vectorization operator. The matrix ${H}_{\mathsf{img}}$ is given by
\begin{equation*}
    {H}_{\mathsf{img}} = \big({X}_{T}^{\top} \otimes {I}_{N K_{\mathsf{RX}}} \big) \big({P}_{\mathsf{TX}} \ast {P}_{\mathsf{RX}} \big),
\end{equation*}
where $\otimes$ and $\ast$ denote the Kronecker and column-wise Khatri-Rao products, and ${I}_{n}$ denotes the identity matrix of size $n \times n$. Matrices ${P}_{\mathsf{RX}}$, ${H}_{\mathsf{comm}}$ and ${Y}_{T}$ are concatenations of local path delay, channel and received symbol matrices across all $N$ base stations.

%${P}_{\mathsf{RX}}^{\top} & = \begin{bmatrix}
%\big({P}_{\mathsf{RX}}^{(1)}\big)^{\top} & \cdots & \big({P}_{\mathsf{RX}}^{(N)}\big)^{\top}
%\end{bmatrix}, \\
%{H}_{\mathsf{comm}}^{\top} & = \begin{bmatrix}
%\big({H}_{\mathsf{comm}}^{(1)}\big)^{\top} & \cdots & \big({H}_{\mathsf{comm}}^{(N)}\big)^{\top}
%\end{bmatrix}, \\
%{Y}_{T}^{\top} & = \begin{bmatrix}
%\big({Y}_{T}^{(1)}\big)^{\top} & \cdots & \big({Y}_{T}^{(N)}\big)^{\top}
%\end{bmatrix},$

%The optimal values of ${f}$ and ${X}_{T-T_{1}}$ in~(\ref{eq:opt3}) and~(\ref{eq:opt4}) are coupled with each other via the matrices ${H}_{\mathsf{img}}$ and ${H}_{\mathsf{comm}}$. This motivates using an \emph{alternating} procedure for solving~\eqref{prb:1} and~\eqref{prb:2}, that alternates between recovering ${f}$ while keeping ${X}_{T-T_{1}}$ fixed, and vice-versa. We shall expand upon this observation in Section~\ref{subsec:results_algo}, where we propose an ADMM-based algorithm for solving~\eqref{prb:2}.

%The coupled nature of~(\ref{eq:opt3}) and~(\ref{eq:opt4}) makes further simplification difficult.

\begin{algorithm}[tb]
    \caption{\emph{Distributed Simultaneous Imaging \& Symbol Detection} (DSISD)}
    \label{alg:admm_dist}
    \textbf{Input:}~${P}_{\mathsf{TX}}$,~${P}_{\mathsf{RX}}^{(n)}$,~${Y}_{T}^{(n)}$,~$\mathcal{X}_{T-T_{1}}$,~${X}_{T_{1}}$,~$K$,~$\rho_{X}$,~$\rho_{f}$
\begin{algorithmic}[1]
   \FOR{node $n=1$ {\bfseries to} $N$ in $\mathcal{V}$ \COMMENT{in parallel}}
   \STATE Initialize ${f}_{0}^{(n)} = {D}_{f,0}^{(n)} = {0},{X}_{T-T_{1},0}^{(n)} = {D}_{X,0}^{(n)} = {0}$
   \FOR{iteration $k=1$ {\bfseries to} $K$}
   \STATE Transmit ${f}_{k-1}^{(n)}$, ${X}_{T-T_{1},k-1}^{(n)}$ to $\big\{m: (n,m) \in \mathcal{E}\big\}$
   \STATE Receive $\big\{{f}_{k-1}^{(m)},~{X}_{T-T_{1},k-1}^{(m)},~\forall m: (n,m) \in \mathcal{E}\big\}$
   %\IF{node $n \in \left\{1,\cdots,N\right\}$}
   \STATE Update reflectivities ${f}_{k}^{(n)}$ by solving
   \begin{equation*}
        \min_{{f}} \left\{
        \begin{aligned}
            &\resizebox{.65\hsize}{!}{$\frac{\rho_{f}}{2} \big\| \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {f}_{k-1}^{(m)} {+} {L}_{\mathcal{G}}(n,n) {f} {+} {D}_{f,k-1}^{(n)} \big\|_{2}^{2}$} \\ &\resizebox{.65\hsize}{!}{${+} \frac{1}{2} \big\|{Y}_{T}^{(n)} {-} {P}_{\mathsf{RX}}^{(n)} \mathsf{diag}\big({f}\big) \big({P}_{\mathsf{TX}} \big)^{\top} {X}_{T,k-1}^{(n)} \big\|_{F}^{2}$}
        \end{aligned}\right\}
   \end{equation*}
   \STATE Update uplink symbols ${X}_{T-T_{1},k}^{(n)}$ by solving
   \begin{equation*}
        \min_{{X}} \left\{
        \begin{aligned}
            &\resizebox{.65\hsize}{!}{$\frac{\rho_{X}}{2} \big\| \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {X}_{T-T_{1},k-1}^{(m)} {+} {L}_{\mathcal{G}}(n,n) {X} {+} {D}_{X,k-1}^{(n)} \big\|_{2}^{2}$} \\ &\resizebox{.65\hsize}{!}{${+} \frac{1}{2} \big\|{Y}_{T}^{(n)} {-} {P}_{\mathsf{RX}}^{(n)} \mathsf{diag}\big({f}_{k}^{(n)}\big) \big({P}_{\mathsf{TX}} \big)^{\top} {X} \big\|_{F}^{2}$}
        \end{aligned}\right\}
   \end{equation*}
   %\ELSIF{$n = N$}
   %\STATE Update reflectivities ${f}_{k}^{(n)}$ by solving
   %\begin{equation*}
    %    \min_{{f}} \bigg\{\resizebox{.65\hsize}{!}{$\frac{\rho_{f}}{2} \big\| \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {f}_{k-1}^{(m)} + {L}_{\mathcal{G}}(n,n) {f} + {D}_{f,k-1}^{(n)} \big\|_{2}^{2}$}\bigg\}
   %\end{equation*}
   %\STATE Update uplink symbols ${X}_{T-T_{1},k}^{(n)}$ by solving
   %\begin{equation*}
   %     \min_{{X}} \left\{
    %    \begin{aligned}
    %        &\resizebox{.65\hsize}{!}{$\frac{\rho_{X}}{2} \big\| \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {X}_{T-T_{1},k-1}^{(m)} + {L}_{\mathcal{G}}(n,n) {X} + {D}_{X,k-1}^{(n)} \big\|_{2}^{2}$} \\ &+ I_{\mathcal{X}_{T-T_{1}}}\big({X}\big)
     %   \end{aligned}\right\}
   %\end{equation*}
   %\ENDIF
   \STATE Update dual variables via
   \begin{align*}
       &\resizebox{.75\hsize}{!}{${D}_{f,k}^{(n)} = {D}_{f,k-1}^{(n)} {+} \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {f}_{k}^{(m)} {+} {L}_{\mathcal{G}}(n,n) {f}_{k}^{(n)}$} \\
       &\resizebox{.85\hsize}{!}{${D}_{X,k}^{(n)} = {D}_{X,k-1}^{(n)} {+} \sum\limits_{m} {L}_{\mathcal{G}}(n,m) {X}_{T-T_{1},k}^{(m)} {+} {L}_{\mathcal{G}}(n,n) {X}_{T-T_{1},k}^{(n)}$}
   \end{align*}
   \ENDFOR
   \ENDFOR
   \STATE \textbf{Output:} $\hat{{f}} = {f}_{K}^{(N)}$, $\hat{{X}}_{T-T_{1}} = \Pi_{\mathcal{X}_{T-T_{1}}}\big({X}_{T-T_{1},K}^{(N)}\big)$
\end{algorithmic}
\end{algorithm}

Note that the values of~\eqref{eq:opt3} and~\eqref{eq:opt4} are coupled. In the following lemma, we characterize conditions under which stationary points satisfying~(\ref{eq:opt3}) and~(\ref{eq:opt4}) are \emph{decoupled}.% . %Hence, any pair $({f}^{*},{X}_{T-T_{1}}^{*})$ that satisfies~(\ref{eq:opt3}) and~(\ref{eq:opt4}) is a valid stationary point. 

%\textcolor{red}{decoupled or decoupled?}

%\textcolor{red}{Do not number equations you are not referring to in the text}

\begin{lemma}
    \label{lmm:1}
    Let ${N}_{T} = {0}$. If ${X}_{T_{1}} \big({X}_{T_{1}}^{*}\big)^{\dagger} = {I}_{K_{\mathsf{TX}}}$, or equivalently, $T_{1} \geq K_{\mathsf{TX}}$ for time-orthogonal pilots, then~\eqref{eq:opt3} and~\eqref{eq:opt4} are decoupled.
\end{lemma}
\begin{proof}
In the absence of noise, ${f}^{*}$ from~\eqref{eq:opt3} is given by
\begin{equation*}
    \resizebox{.99\hsize}{!}{${f}^{*} = \big({P}_{\mathsf{TX}} \ast {P}_{\mathsf{RX}} \big)^{\dagger} \big(\big({X}_{T} \big({X}_{T}^{*}\big)^{\dagger}\big)^{\top} \otimes {I}_{N K_{\mathsf{RX}}} \big) \big({P}_{\mathsf{TX}} \ast {P}_{\mathsf{RX}} \big) {f}.$}
\end{equation*}

The above expression is decoupled with the recovered uplink symbols ${X}_{T}^{*}$ when ${X}_{T} \big({X}_{T}^{*}\big)^{\dagger} = {I}_{K_{\mathsf{TX}}}$. Since data portion of ${X}_{T}$ and recovered symbols ${X}_{T}^{*}$ may differ, a sufficient condition is thus ${X}_{T_{1}} \big({X}_{T_{1}}^{*}\big)^{\dagger} = {I}_{K_{\mathsf{TX}}}$. For time-orthogonal pilot symbols, this condition is equivalent to
\begin{equation*}
    \mathsf{rank}\big({X}_{T_{1}}\big) = \min\big\{T_{1},K_{\mathsf{TX}}\big\} \geq K_{\mathsf{TX}} \implies T_{1} \geq K_{\mathsf{TX}}.
\end{equation*}
\end{proof}

%Note that although the data portion of the transmitted symbols, the first $T_{1}$ pilot symbols are the same in both ${X}_{T}$ and ${X}_{T}^{*}$ since the pilots are known a-priori to all base stations. Hence, a sufficient condition for ${X}_{T} \big({X}_{T}^{*}\big)^{\dagger} = {I}_{K_{\mathsf{TX}}}$ is

Following Lemma~\ref{lmm:1}, we assume $T_{1} = K_{\mathsf{TX}}$ in all subsequent discussion. We now present the proposed DSISD algorithm for solving~\eqref{prb:2}.

%which also equals the pilot duration that maximizes MIMO communication rate, e.g., see~\cite{Tse2002,Hassibi2003}. %Hence, Lemma~\ref{lmm:1} implies that imaging functionality can be incorporated ``for free'' with no changes to existing communication infrastructure. We refer the reader to our previous work in~\cite{Mehrotra2021a,Mehrotra2021b} for a more detailed information-theoretic treatment.

\subsection{Distributed Simultaneous Imaging \& Symbol Detection}
\label{subsec:results_algo}

The bi-convexity of the objective function $\mathcal{L}\big({f},{X}_{T-T_{1}}\big)$ naturally motivates using an \emph{alternating} procedure to solve~\eqref{prb:2}. The proposed DSISD algorithm (Algorithm~\ref{alg:admm_dist}) is thus based on consensus ADMM~\citep{Boyd2011}. 

Let the concatenation of local solutions across all $N$ nodes be denoted by variables \mbox{$\overline{{X}}^{\top} = \big[\big({X}_{T-T_{1}}^{(1)}\big)^{\top},\cdots,\big({X}_{T-T_{1}}^{(N)}\big)^{\top} \big]$} and \mbox{$\overline{{f}}^{\top} = \big[\big({f}^{(1)}\big)^{\top},\cdots,\big({f}^{(N)}\big)^{\top}\big]$}. Moreover, let
\begin{equation*}
    \resizebox{.99\hsize}{!}{$g\big(\overline{{X}},\overline{{f}}\big) = \frac{1}{2} \sum\limits_{n = 1}^{N}\big\|{Y}_{T}^{(n)} {-} {P}_{\mathsf{RX}}^{(n)} \mathsf{diag}\big({f}^{(n)}\big) \big({P}_{\mathsf{TX}} \big)^{\top} {X}_{T}^{(n)} \big\|_{F}^{2}$}
\end{equation*}
denote the objective function in~\eqref{prb:2}. Finally, \mbox{${L}_{\mathcal{G}} \in \mathbb{R}^{N \times N}$} denotes the Laplacian matrix for $\mathcal{G}$. %Per Assumption~\ref{assumpn:5}, every node knows its corresponding row in Laplacian matrix ${L}_{\mathcal{G}}$.

With above defined notation,~\eqref{prb:2} may be recast as
\begin{align}
    \label{prb:3}
    &\min_{\overline{{X}},\overline{{f}}} g\big(\overline{{X}},\overline{{f}}\big) \nonumber \\
    &\text{s.t.}~\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} = {0},~\big({L}_{\mathcal{G}} \otimes {I}_{M} \big)  \overline{{f}} = {0}.
    \tag{P3}
\end{align}

At every iteration $k \in \{0,1,\cdots\}$, DSISD performs the following ADMM updates:
\begin{align}
    \label{eq:alg1}
    \overline{{f}}^{k+1} &= \arg\min_{\overline{{f}}} \mathcal{A}\big(\overline{{X}}^{k},\overline{{f}},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big),
    \tag{A1} \\
    \label{eq:alg2}
    \overline{{X}}^{k+1} &= \resizebox{.55\hsize}{!}{$\arg\min\limits_{\overline{{X}}} \mathcal{A}\big(\overline{{X}},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big),$}
    \tag{A2} \\
    \label{eq:alg3}
    \overline{{D}}_{f}^{k+1} &= \overline{{D}}_{f}^{k} {+} \big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}}^{k+1}.
    \tag{A3} \\
    \label{eq:alg4}
    \overline{{D}}_{X}^{k+1} &= \overline{{D}}_{X}^{k} {+} \big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}}^{k+1},
    \tag{A4}
\end{align}
where $\mathcal{A}\big(\overline{{X}},\overline{{f}},\overline{{D}}_{X},\overline{{D}}_{f}\big)$ denotes the augmented Lagrangian,
\begin{multline*}
    \mathcal{A}\big(\overline{{X}},\overline{{f}},\overline{{D}}_{X},\overline{{D}}_{f}\big) = g\big(\overline{{X}},\overline{{f}}\big) {+} \frac{\rho_{f}}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}} \big\|_{F}^{2} \\
    {+} \rho_{X} \left\langle \overline{{D}}_{X}, \big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} \right\rangle {+} \rho_{f} \left\langle \overline{{D}}_{f}, \big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}} \right\rangle \\ {+} \frac{\rho_{X}}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} \big\|_{F}^{2}.
    %\mathcal{A}\big(\overline{{X}},\overline{{f}},\overline{{D}}_{X},\overline{{D}}_{f}\big) = g\big(\overline{{X}},\overline{{f}}\big) + \\ \resizebox{.875\hsize}{!}{$\frac{\rho_{X}}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} + \overline{{D}}_{X}\big\|_{F}^{2} + \frac{\rho_{f}}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}} + \overline{{D}}_{f}\big\|_{F}^{2},$}
\end{multline*}

The variables $\overline{{D}}_{X}$ and $\overline{{D}}_{f}$ denote scaled dual variables, whereas $\rho_{X}$ and $\rho_{f}$ denote penalty parameters.

The updates in~(\ref{eq:alg1}) to~(\ref{eq:alg4}) can be performed locally at every base station since $g\big(\overline{{X}},\overline{{f}}\big)$ and $\mathcal{A}\big(\overline{{X}},\overline{{f}},\overline{{D}}_{X},\overline{{D}}_{f}\big)$ are separable across pairs of local solutions $\big({f}^{(n)},{X}_{T}^{(n)}\big)$. Below, we derive performance guarantees for DSISD. %At every iteration, nodes (i) transmit local solutions to neighbors, (ii) receive local solutions from neighbors, and (iii) update local solutions and dual variables via~(\ref{eq:alg1}) to~(\ref{eq:alg4}).  Note that DSISD solves the original integer-constrained problem in~\eqref{prb:2}, and does not make any approximations on ${X}_{T-T_{1}}$.

%Besides local knowledge, see Assumptions~\ref{assumpn:4} and~\ref{assumpn:5}, every node requires knowledge of the updates of neighboring nodes. Hence, 

\subsection{Performance Guarantees for DSISD}
\label{subsec:results_algo_perf}

In Theorem~\ref{thm:1} and Corollary~\ref{corr:1}, we characterize convergence guarantees and algorithm complexity for DSISD. %To derive convergence guarantees, we make the same unconstrained relaxation as made in Section~\ref{subsec:results_opt_condn}.
\\
\begin{theorem}
\label{thm:1}
Let Assumptions~\ref{assumpn:1},~\ref{assumpn:4},~\ref{assumpn:5} and the conditions in Lemma~\ref{lmm:1} hold. Then, the updates of DSISD satisfy the following properties:

\textbf{Asymptotic consensus:} All $N$ nodes in $\mathcal{G}$ are in consensus asymptotically, i.e.,
\begin{align*}
    \lim_{k \rightarrow \infty} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}}^{k+1}\big\|_{2} &= 0, \\
    \lim_{k \rightarrow \infty} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}}^{k+1}\big\|_{F} &= 0.  
\end{align*}

\textbf{Convergence to stationary points:} Limit points of iterates $\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big)$ converge to a KKT point of~\eqref{prb:3}.

\textbf{Sublinear convergence rate:} Iterates $\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big)$ converge to a KKT point of~\eqref{prb:3} with rate $O\big({1}/{K}\big)$ in terms of the optimality gap
\begin{multline*}
    Q\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big) = \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}}^{k+1}\big\|_{F}^{2} {+} \\ \big\|\nabla_{\overline{{f}}} \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big) \big\|_{F}^{2} {+} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}}^{k+1}\big\|_{2}^{2} \\ {+} \big\|\nabla_{\overline{{X}}} \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big) \big\|_{F}^{2}.
\end{multline*}
\end{theorem}

\begin{proof}
We prove the three desired results individually.

\textbf{Result~$1$: Asymptotic Consensus}

We seek to prove
\begin{equation*}
    \lim_{k \rightarrow \infty} \big\|\overline{{D}}_{f}^{k+1}{-}\overline{{D}}_{f}^{k} \big\|_{2} = 0,~\lim_{k \rightarrow \infty} \big\|\overline{{D}}_{X}^{k+1}{-}\overline{{D}}_{X}^{k} \big\|_{2} = 0.
\end{equation*}
%as per steps~(\ref{eq:alg3} and~(\ref{eq:alg4}) of DSISD.

We show the above result via two intermediate steps.

\textbf{Step~$1$:} We first derive upper bounds on successive dual update norms, $\big\|\overline{{D}}_{f}^{k+1}{-}\overline{{D}}_{f}^{k} \big\|_{2}$ and $\big\|\overline{{D}}_{X}^{k+1}{-}\overline{{D}}_{X}^{k} \big\|_{2}$. Consider the first-order optimality condition for~\eqref{eq:alg2},
\begin{equation*}
    \nabla_{\overline{{X}}} g\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\big) {+} \rho_{X} \big({L}_{\mathcal{G}}^{\top} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{D}}_{X}^{k+1} = {0}.
\end{equation*}
Thus, an upper bound on $\big\|\overline{{D}}_{X}^{k+1} {-} \overline{{D}}_{X}^{k} \big\|_{F}^{2}$ is given by
\begin{equation*}
    \resizebox{.99\hsize}{!}{$\big\| \overline{{D}}_{X}^{k+1} {-} \overline{{D}}_{X}^{k} \big\|_{F}^{2} \leq \frac{\nicefrac{1}{\rho_{X}^{2}}}{\lambda_{\mathsf{min}}\big({L}_{\mathcal{G}}^{\top} {L}_{\mathcal{G}}\big)} \big\| \nabla_{\overline{{X}}} g\big(\overline{{X}}^{k},\overline{{f}}^{k}\big) {-} \nabla_{\overline{{X}}} g\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\big) \big\|_{F}^{2}$},
\end{equation*}
where we have used the fact that $\frac{1}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} \big\|_{F}^{2}$ is $\lambda_{\mathsf{min}}\big({L}_{\mathcal{G}}^{\top} {L}_{\mathcal{G}}\big)$-strongly convex.

%On appropriate substitutions, the right hand side can be upper bounded in terms of successive \emph{primal} update norms, $\big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2}$, $\big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{F}^{2}$. Thus, we next show $\lim_{k \rightarrow \infty} \big\|\overline{{f}}^{k+1} {-} \overline{{f}}^{k}\big\|_{2} = 0$ and $\lim_{k \rightarrow \infty} \big\|\overline{{X}}^{k+1} {-} \overline{{X}}^{k}\big\|_{F} = 0$.

The right hand side of the inequality may be written as
\begin{multline*}
    \big\| \nabla_{\overline{{X}}} g\big(\overline{{X}}^{k},\overline{{f}}^{k}\big) {-} \nabla_{\overline{{X}}} g\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\big) \big\|_{F}^{2} = \\ \sum\limits_{n = 1}^{N} \big\|\big({H}_{\mathsf{comm},k}^{(n)}\big)^{H} \big({H}_{\mathsf{comm},k}^{(n)} {X}_{T-T_{1},k}^{(n)} - {Y}_{T-T_{1}}^{(n)} \big) {-} \\ \big({H}_{\mathsf{comm},k+1}^{(n)}\big)^{H} \big({H}_{\mathsf{comm},k+1}^{(n)} {X}_{T-T_{1},k+1}^{(n)} - {Y}_{T-T_{1}}^{(n)}\big) \big\|_{F}^{2}.
\end{multline*}

On substituting the expression for ${H}_{\mathsf{comm},k}^{(n)}$~(c.f., \eqref{eq:sys1}), the term inside the summation above may be upper bounded in terms of successive \emph{primal} update norms, $\big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2}$ and $\big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{F}^{2}$, as
\begin{multline*}
    4 \cdot \left\Vert \left({H}_{\mathsf{comm},k}^{(n)}\right)^{H} \cdot {H}_{\mathsf{comm},k}^{(n)} \cdot \left({X}_{T-T_{1},k}^{(n)} - {X}_{T-T_{1},k+1}^{(n)}\right) \right\Vert_{F}^{2} \\ \resizebox{.99\hsize}{!}{$+ 4 \cdot \left\Vert \left(\left({H}_{\mathsf{comm},k}^{(n)}\right)^{H} \cdot {H}_{\mathsf{comm},k}^{(n)} - \left({H}_{\mathsf{comm},k}^{(n)}\right)^{H} \cdot {H}_{\mathsf{comm},k+1}^{(n)}\right) \cdot {X}_{T-T_{1},k+1}^{(n)} \right\Vert_{F}^{2}$} \\ \resizebox{.99\hsize}{!}{$+ 4 \cdot \left\Vert \left(\left({H}_{\mathsf{comm},k}^{(n)}\right)^{H} \cdot {H}_{\mathsf{comm},k+1}^{(n)} - \left({H}_{\mathsf{comm},k+1}^{(n)}\right)^{H} \cdot {H}_{\mathsf{comm},k+1}^{(n)}\right) \cdot {X}_{T-T_{1},k+1}^{(n)} \right\Vert_{F}^{2}$} \\ + 4 \cdot \left\Vert \left(\left({H}_{\mathsf{comm},k}^{(n)}\right)^{H} - \left({H}_{\mathsf{comm},k+1}^{(n)}\right)^{H} \right) \cdot {Y}_{T-T_{1}}^{(n)} \right\Vert_{F}^{2},
\end{multline*}
where recall that ${H}_{\mathsf{comm},k}^{(n)} = {P}_{\mathsf{RX}}^{(n)} \mathsf{diag}\big({f}_{k}^{(n)}\big) \big({P}_{\mathsf{TX}} \big)^{\top}$.

Similarly, $\big\| \overline{{D}}_{f}^{k+1} {-} \overline{{D}}_{f}^{k} \big\|_{F}^{2}$ is also upper bounded in terms of the primal update norms. Therefore, to show the desired result, it suffices to show $\lim_{k \rightarrow \infty} \big\|\overline{{f}}^{k+1} {-} \overline{{f}}^{k}\big\|_{2} = 0$ and $\lim_{k \rightarrow \infty} \big\|\overline{{X}}^{k+1} {-} \overline{{X}}^{k}\big\|_{F} = 0$.

\textbf{Step~$2$:} We equivalently show $\sum\limits_{k = 1}^{\infty} \big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2} < \infty$ and $\sum\limits_{k = 1}^{\infty} \big\| \overline{{f}}^{k+1} - \overline{{f}}^{k} \big\|_{2}^{2} < \infty$ via two sub-results. 

(i) First, we show that the augmented Lagrangian is upper bounded in terms of the primal update norms as
\begin{multline*}
    \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) {-} \mathcal{A}\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) \\ \resizebox{.99\hsize}{!}{$\leq {-}\frac{ \lambda_{\mathsf{min}}\big({L}_{\mathcal{G}}^{\top} {L}_{\mathcal{G}}\big)}{2} \big(\rho_{X} \big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2} {+} \rho_{f} \big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{2}^{2} \big).$}
\end{multline*}

%We show the above by upper bounding the left hand side and using the first-order optimality conditions corresponding to~\eqref{eq:alg1} and~\eqref{eq:alg2}, the convexity of the objective function $g\left(\overline{ {X}},\overline{ {f}}\right)$ in $\overline{ {X}}$ (resp. $\overline{ {f}}$) given fixed $\overline{ {f}}$ (resp. $\overline{ {X}}$), as well as the $\lambda_{\mathsf{min}}\big({L}_{\mathcal{G}}^{\top} {L}_{\mathcal{G}}\big)$ strong convexity of the terms $\frac{1}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} \big\|_{F}^{2}$ and $\frac{1}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{M}}} \big) \overline{{f}} \big\|_{2}^{2}$.

We show the above by upper bounding the left hand side,
\begin{equation*}
    \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) {-} \mathcal{A}\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) = A + B,
\end{equation*}
where the terms $A$ and $B$ are given by
\begin{align*}
    A &= \mathcal{A}\big(\overline{ {X}}^{k+1},\overline{ {f}}^{k+1},\overline{ {D}}_{X}^{k},\overline{ {D}}_{f}^{k}\big) {-} \mathcal{A}\big(\overline{ {X}}^{k},\overline{ {f}}^{k+1},\overline{ {D}}_{X}^{k},\overline{ {D}}_{f}^{k}\big), \\
    B &= \mathcal{A}\big(\overline{ {X}}^{k},\overline{ {f}}^{k+1},\overline{ {D}}_{X}^{k},\overline{ {D}}_{f}^{k}\big) {-} \mathcal{A}\big(\overline{ {X}}^{k},\overline{ {f}}^{k},\overline{ {D}}_{X}^{k},\overline{ {D}}_{f}^{k}\big).
\end{align*}

To upper bound $A$ and $B$, we use the first-order optimality conditions corresponding to~\eqref{eq:alg1} and~\eqref{eq:alg2}, e.g., for $A$,
\begin{equation*}
    \resizebox{.99\hsize}{!}{$\left\langle \nabla_{\overline{{X}}} g\left(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\right) + \rho_{X} \left({L}_{\mathcal{G}}^{\top} \otimes {I}_{K_{TX}} \right) \overline{{D}}_{X}^{k+1}, \left(\overline{{X}}^{k+1} - \overline{{X}}\right) \right\rangle \leq 0,~\forall \overline{{X}}.$}
\end{equation*}

Hence, $A$ is upper bounded as
\begin{multline*}
    \resizebox{.99\hsize}{!}{$A \leq g\left(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\right) - g\left(\overline{{X}}^{k},\overline{{f}}^{k+1}\right) + \frac{\rho_{X}}{2} \left\Vert\left({L}_{\mathcal{G}} \otimes {I}_{K_{TX}} \right) \cdot \overline{{X}}^{k+1} \right\Vert_{F}^{2}$} \\
    - \left\langle \nabla_{\overline{{X}}} g\left(\overline{{X}}^{k+1},\overline{{f}}^{k+1}\right), \left(\overline{{X}}^{k+1} - \overline{{X}}^{k}\right) \right\rangle \\ - \rho_{X} \left\langle \left(\left({L}_{\mathcal{G}}^{\top} \cdot {L}_{\mathcal{G}} \right) \otimes {I}_{K_{TX}} \right) \overline{{X}}^{k+1}, \left(\overline{{X}}^{k+1} - \overline{{X}}^{k}\right) \right\rangle.
\end{multline*}

Invoking the convexity of the objective function $g\left(\overline{ {X}},\overline{ {f}}\right)$ in $\overline{ {X}}$ given fixed $\overline{ {f}}$, as well as the $\lambda_{\mathsf{min}}\big({L}_{\mathcal{G}}^{\top} {L}_{\mathcal{G}}\big)$ strong convexity of $\frac{1}{2} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}} \big\|_{F}^{2}$, we obtain
\begin{equation*}
    A \leq -\frac{\rho_{X} \cdot \lambda_{\mathsf{min}}\left({L}_{\mathcal{G}}^{\top} \cdot {L}_{\mathcal{G}}\right)}{2} \cdot \left\Vert \overline{{X}}^{k+1} - \overline{{X}}^{k} \right\Vert_{F}^{2}.
\end{equation*}

Similarly, $B$ is upper bounded as
\begin{equation*}
    B \leq -\frac{\rho_{f} \cdot \lambda_{\mathsf{min}}\left({L}_{\mathcal{G}}^{\top} \cdot {L}_{\mathcal{G}}\right)}{2} \cdot \left\Vert \overline{{f}}^{k+1} - \overline{{f}}^{k} \right\Vert_{F}^{2}.
\end{equation*}

Hence, we obtain the desired result.

(ii) Next, we show that the augmented Lagrangian is lower bounded at every iteration, i.e.,
\begin{align*}
    &\sum\limits_{k = 1}^{K}  \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) > -\infty, \\
    & \sum\limits_{k = 1}^{K} \mathcal{A}\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) > -\infty.
\end{align*}

To show the above result, recall from~\eqref{eq:alg3} and~\eqref{eq:alg4} that the dual updates satisfy
\begin{align*}
    \left({L}_{\mathcal{G}} \otimes {I}_{K_{TX}} \right) \cdot \overline{{X}}^{k+1} &= \overline{{D}}_{X}^{k+1} - \overline{{D}}_{X}^{k}, \\ \left({L}_{\mathcal{G}} \otimes {I}_{M} \right) \cdot \overline{{f}}^{k+1} &= \overline{{D}}_{f}^{k+1} - \overline{{D}}_{f}^{k}.
\end{align*}

Furthermore, note that for any $C$ and $D$, we have
\begin{equation*}
    \big\langle C,D \big\rangle = \frac{1}{2} \bigg(\big\|C+D \big\|_{F}^{2} - \big\|C \big\|_{F}^{2} - \big\|D \big\|_{F}^{2}\bigg).
\end{equation*}

On appropriate substitutions, we obtain the desired result.

On taking the limit $K \rightarrow \infty$ in (i) and (ii) above, we obtain $\sum\limits_{k = 1}^{\infty} \big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2} < \infty$ and $\sum\limits_{k = 1}^{\infty} \big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{2}^{2} < \infty$.

\textbf{Result~$2$: Convergence to Stationary Points}

The KKT conditions corresponding to~\eqref{prb:3} are
\begin{gather*}
    \nabla_{\overline{{X}}} g\big(\overline{{X}}^{*},\overline{{f}}^{*}\big) {+} \rho_{X} \big({L}_{\mathcal{G}}^{\top} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{D}}_{X}^{*} = {0}, \\
    \nabla_{\overline{{f}}} g\big(\overline{{X}}^{*},\overline{{f}}^{*}\big) {+} \rho_{X} \big({L}_{\mathcal{G}}^{\top} \otimes {I}_{M} \big) \overline{{D}}_{f}^{*} = {0}, \\
    \big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}}^{*} = {0},~\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}}^{*} = {0}.
\end{gather*}

We aim to show that the limit points corresponding to Algorithm~\ref{alg:admm_dist} satisfy the above KKT conditions. To that end, observe that in the limit $k \rightarrow \infty$, the update steps~(\ref{eq:alg1}) and~(\ref{eq:alg2}) satisfy
\begin{gather*}
    \resizebox{.99\hsize}{!}{$\nabla_{\overline{{X}}} \mathcal{A} = {0} \implies \nabla_{\overline{{X}}} g\big(\overline{{X}}^{*},\overline{{f}}^{*}\big) {+} \rho_{X} \big({L}_{\mathcal{G}}^{\top} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{D}}_{X}^{*} = {0},$} \\
    \resizebox{.99\hsize}{!}{$\nabla_{\overline{{f}}} \mathcal{A} = {0} \implies \nabla_{\overline{{f}}} g\big(\overline{{X}}^{*},\overline{{f}}^{*}\big) {+} \rho_{f} \big({L}_{\mathcal{G}}^{\top} \otimes {I}_{M} \big) \overline{{D}}_{f}^{*} = {0}.$}
\end{gather*}

In addition, since $\lim_{k \rightarrow \infty} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{M} \big) \overline{{f}}^{k+1}\big\|_{2} = 0$ and $\lim_{k \rightarrow \infty} \big\|\big({L}_{\mathcal{G}} \otimes {I}_{K_{\mathsf{TX}}} \big) \overline{{X}}^{k+1}\big\|_{F} = 0$ (c.f., Result~$1$), convergence to stationary points follows.

\textbf{Result~$3$: Sublinear Convergence Rate}

To derive convergence rates, we bound the optimality gap defined in the theorem statement. Per Result~$1$, for large enough $\xi > 0$, the optimality gap is upper bounded as
\begin{equation*}
    \resizebox{.99\hsize}{!}{$Q\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big) \leq \xi \big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2} {+} \xi \big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{F}^{2}.$}
\end{equation*} 

Moreover, for some large enough $\nu > 0$, Result~$1$ implies
\begin{multline*}
    \mathcal{A}\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) {-} \mathcal{A}\big(\overline{{X}}^{k},\overline{{f}}^{k},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k}\big) \\ \leq {-}\nu \big\| \overline{{X}}^{k+1} {-} \overline{{X}}^{k} \big\|_{F}^{2} {-} \nu \big\| \overline{{f}}^{k+1} {-} \overline{{f}}^{k} \big\|_{F}^{2}.
\end{multline*}

On averaging over indices $k = 1, \cdots, K$, we obtain
\begin{multline*}
    \frac{1}{K} \sum\limits_{k = 1}^{K} Q\big(\overline{{X}}^{k+1},\overline{{f}}^{k+1},\overline{{D}}_{X}^{k},\overline{{D}}_{f}^{k} \big) \leq \\ \frac{\xi}{K \nu} \big(\mathcal{A}\big(\overline{{X}}^{1},\overline{{f}}^{1},\overline{{D}}_{X}^{1},\overline{{D}}_{f}^{1}\big) {-} \mathcal{A}\big(\overline{{X}}^{K+1},\overline{{f}}^{K+1},\overline{{D}}_{X}^{1},\overline{{D}}_{f}^{1}\big) \big).
\end{multline*}

In other words, the convergence in terms of the optimality gap is sublinear with rate $O\big({1}/{K}\big)$.
\end{proof}

\begin{remark}
To the best of our knowledge, we are not aware of any existing convergence analysis for ADMM that is directly applicable to our problem, which is distributed, integer constrained, bi-convex, and non-separable. On the one hand, in~\citep{Yin2013}, the authors consider the \emph{centralized} bi-convex and non-separable function class and show sublinear convergence assuming the objective function satisfies the Kurdyka–\L ojasiewicz (KL) inequality. On the other hand, in~\citep{Razaviyayn2016}, the authors consider the distributed non-convex but \emph{separable} function class and show convergence to stationary points. Neither analysis applies to our problem. However, in the absence of integer constraints, our problem is closely related to matrix factorization (MF). Hence, we have adapted prior convergence analysis for MF~\citep{Hajinezhad2016,Hajinezhad2018,Hong2017} to our problem. Since our problem is not identical to MF, our results have certain minor differences. Specifically, convergence to stationary points for MF only holds under certain regimes on the ADMM penalty parameters (e.g., $\rho > 1)$. No such conditions are required in our results.
\end{remark}

\begin{remark}
We remark that the applicability of ADMM to bi-convex problems is well-known from~\citep{Boyd2011}. Since strong duality does not hold in bi-convex problems, we can only demonstrate approximate convergence to KKT points. To do so, we have used the optimality gap function from~\citep{Hajinezhad2016,Hajinezhad2018,Hong2017} since it quantifies both first-order optimality conditions and the consensus error.
\end{remark}

We now characterize the algorithm complexity for DSISD.% in the following corollary.
\\
\begin{corollary}
    \label{corr:1}
    Let the same assumptions as in Theorem~\ref{thm:1} hold, and let $\epsilon > 0$ be a desired accuracy. Then, the algorithm complexity for DSISD is $O\big(2 |\mathcal{E}| \big(M {+} K_{\mathsf{TX}} (T{-}T_{1}) + \big(M{+}K_{\mathsf{RX}} T\big) \big({M N K_{\mathsf{RX}} T}\big)\big)/{\epsilon}\big)$.
\end{corollary}

\begin{proof}
The communication complexity is given by
\begin{equation*}
    O\big(2 |\mathcal{E}| \big(M {+} K_{\mathsf{TX}} (T{-}T_{1}) \big)/{\epsilon}\big),
\end{equation*}
which corresponds to the total number of real entries transferred across the network $\mathcal{G}$ over $K = O\big({1}/{\epsilon}\big)$ iterations as per the convergence rate in Theorem~\ref{thm:1}.

The computational complexity corresponds to the total cost of least-squares updates in every iteration and equals
\begin{equation*}
    O\big(N \big(M \big(K_{\mathsf{RX}}T\big)^{2} {+} M^{2} K_{\mathsf{RX}}T {+} K_{\mathsf{RX}} K_{\mathsf{TX}}^{2} {+} K_{\mathsf{TX}} K_{\mathsf{RX}}^{2} \big)/{\epsilon}\big).
\end{equation*}

Assuming the number of scatterers in the scene largely dominates the number of transmitting or receiving antennas, i.e., $M \gg K_{\mathsf{TX}},~K_{\mathsf{RX}}$, the algorithm complexity is given by the statement in the corollary.
\end{proof}

\begin{figure}[t]
    \centering
    \begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[page=1,width=0.95\linewidth]{setup.pdf}
    \caption{}
    \label{fig:plts_a}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[page=1,width=0.95\linewidth]{q_admm.pdf}
    \caption{}
    \label{fig:plts_b}
    \end{subfigure}
    \caption{(a) Simulated configuration. (b) DSISD converges sublinearly in terms of optimality gap $Q$ for high receive signal-to-noise ratio (SNR) values.}
    \label{fig:plts1}
\end{figure}

For comparison, consider decode-and-image. The communication complexity corresponds to every node transferring its $K_{\mathsf{RX}} \times T$ matrix of received symbols $Y_{T}^{(n)}$ to the central server, and thus equals $O(N K_{\mathsf{RX}} T)$. The computational complexity corresponds to least-squares updates over $N \times$ larger matrices, and equals $O(K_{\mathsf{RX}} N T M (M + K_{\mathsf{RX}} N T))$. Hence, DSISD has $O(N)$ smaller computational complexity compared to decode-and-image.
%, which has complexity \mbox{$O\big(\big(M{+}NK_{\mathsf{RX}} T\big) \big({M N K_{\mathsf{RX}} T}/{\epsilon}\big)\big)$}. We see that DSISD has $O(N)$ smaller total complexity compared to decode-and-image. The primary gains are in the computational complexity, since all $N$ nodes perform local least squares updates in parallel in DSISD on $\nicefrac{1}{N} \times$ lower dimensional data. Since least squares updates have complexity $O\big(m n^{2} + n m^{2}\big)$, for problem dimension $m \times n$, the desired result follows immediately.

In the next section, we numerically evaluate the performance of DSISD and compare it with decode-and-image.

%\textcolor{red}{Is this a Lemma or more like a Corollary}

%To compare the two communication costs from Lemma~\ref{lmm:1}, let us consider two extreme backhaul network topologies: (i) fully connected topology, where $|\mathcal{E}| = \frac{NN}{2}$, and (ii) star topology, where $|\mathcal{E}| = N$. In Fig.~\ref{fig:admm_cost}, we compare the communication costs from Lemma~\ref{lmm:1} for both network topologies for a system configuration with parameters: coherence interval $T = 100$, number of transmit antennas $K_{\mathsf{TX}} = 4$, number of pilots $T_{1} = 4$, number of scatterers in imaging scene $M = 10^{3}$, number of receive antennas per node $K_{\mathsf{RX}} = 64$, number of iterations $K = 10$. In the worst-case with a fully connected backhaul network, Algorithm~\ref{alg:admm_dist} is more communication-efficient than centralized algorithms for networks with up to $N = 4$ base stations. However, in most practical deployments, the number of backhaul links scale linearly with the number of nodes in the network, e.g., star or ring topology. In such scenarios, as shown in Fig.~\ref{fig:admm_cost}, the communication cost of Algorithm~\ref{alg:admm_dist} is $\approx 2.5 \times$ smaller than the centralized problem.

%\begin{Fig.}
%    \centering
%    \includegraphics[page=2,width=0.8\linewidth]{Fig.s_ADMM_Img_Comm1.pdf}
%    \caption{Comparison of communication cost (number of real numbers sent over backhaul network) for Algorithm~\ref{alg:admm_dist} and centralized problem~\eqref{prb:1}. For fully connected backhaul networks, Algorithm~\ref{alg:admm_dist} is more communication-efficient than centralized algorithms for networks with up to $N = 4$ base stations. In practical scenarios such as star backhaul networks, the communication cost of Algorithm~\ref{alg:admm_dist} is $\approx 2.5 \times$ smaller than the centralized problem.}
%    \label{fig:admm_cost}
%\end{Fig.}
